ColaCare: Enhancing Electronic Health Record Modeling through Large Language Model-Driven Multi-Agent Collaboration

We introduce ColaCare, a framework that enhances Electronic Health Record (EHR) modeling through multi-agent collaboration driven by Large Language Models (LLMs). Our approach seamlessly integrates domain-specific expert models with LLMs to bridge the gap between structured EHR data and text-based reasoning. Inspired by the Multidisciplinary Team (MDT) approach used in clinical settings, ColaCare employs two types of agents: DoctorAgents and a MetaAgent, which collaboratively analyze patient data. Expert models process and generate predictions from numerical EHR data, while LLM agents produce reasoning references and decision-making reports within the MDT-driven collaborative consultation framework. The MetaAgent orchestrates the discussion, facilitating consultations and evidence-based debates among DoctorAgents, simulating diverse expertise in clinical decision-making. We additionally incorporate the Merck Manual of Diagnosis and Therapy (MSD) medical guideline within a retrieval-augmented generation (RAG) module for medical evidence support, addressing the challenge of knowledge currency. Extensive experiments conducted on three EHR datasets demonstrate ColaCare's superior performance in clinical mortality outcome and readmission prediction tasks, underscoring its potential to revolutionize clinical decision support systems and advance personalized precision medicine. All code, case studies and a questionnaire are available at the project website: https://colacare.netlify.app.

==> prompts/complete_prompts/action.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's decision of next action: \\

1. You are an authoritative expert in the medical field. You are organizing a collaborative consultation. Now several general doctors have made analysis and judgments on a patient's condition. Your task is to judge whether everyone has reached a consensus on the diagnosis of the patient based on the analysis statements of each doctor. \\

2. In response to the patient's summary report, several general doctors put forward their own opinions and reasons. 
In each general doctor's statement, they first expressed whether they agreed with the previous summary report and gave the degree of confidence in their own judgment. Then, they further elaborated on their views by stating reasons and listing relevant literature. 
The following are their opinions:
Doctor 0's statement is as following:
Regarding the summary report of the leader expert, I agree with the leader, with high confidence.
The reason to support my statement is announced below:
The patient's condition, as described in the summary report, aligns with the high-risk profile for mortality in patients with End-Stage Renal Disease due to Diabetic Nephropathy. The abnormalities in blood sodium, phosphorus, and albumin, along with uncontrolled blood glucose and high systolic blood pressure, are consistent with the severe complications associated with these conditions as outlined in the provided medical documents.
Doctor 1's statement is as following:
Regarding the summary report of the leader expert, I agree with the leader, with high confidence.
The reason to support my statement is announced below:
The patient's condition aligns with the high-risk profile described in the medical documents. The combination of End-Stage Renal Disease, uncontrolled diabetes, electrolyte imbalances, and hypertension all contribute to a significant risk of mortality.
Doctor 2's statement is as following:
Regarding the summary report of the leader expert, I agree with the leader, with high confidence.
The reason to support my statement is announced below:
The patient's condition, as described in the summary report, aligns with the high-risk profile associated with End-Stage Renal Disease and poorly controlled diabetes. The abnormalities in blood sodium, phosphorus, and albumin, along with the high blood glucose and systolic blood pressure, are consistent with severe complications that increase mortality risk.
 \\

3. Next, you need to judge whether the next round of discussion is needed based on each general doctor's statement. Considering the following four cases:
(1) If all doctors agree with the previous summary report, there is no need to continue the discussion.
(2) If some doctors disagree with the previous report, but they are not confident in their judgment and have not listed convincing evidence, there is no need to continue the discussion.
(3) If some doctors strongly oppose the previous report and you think their evidence is worth discussing, we need to continue the discussion.
(4) If most doctors disagree with the previous report, we need to continue the discussion. \\

5. Please output the following two contents in JSON format:
1. Whether to continue the discussion or not.
2. Explain the reasons for your judgment. \\

6. Here are two examples of the format you should output:
{"Action": "Stop the discussion", "Reason": "All doctors agree with the previous summary report"}.
{"Action": "Continue the discussion", "Reason": "Exist a few experts strongly disagree with the previous summary report"}. \\

7. Respond in JSON format without any additional content: \\

\end{tcolorbox}

==> prompts/complete_prompts/collaborative_doctor_review.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Doctors' Discussion Review: \\

1. doctor_collaboration_system = """You are an experienced medical expert participating in a consultation with several other medical experts for a patient. The leader expert of this consultation has generated a summary report based on all experts' analyses of the patient. Please provide your viewpoint on his opinion. \\

2. Here is the relevant medical knowledge:
Document [0] (Title: Hemodialysis ...
Document [1] (Title: ...
\\

3. Here is the opinion of the leader expert:
In my opinion, the patient has a high risk of mortality. \\

4. Here is the summary report generated by the leader expert:
The patient, a 65-year-old male with End-Stage Renal Disease due to Diabetic Nephropathy and Diabetes, exhibits significant clinical markers of severe renal dysfunction and metabolic imbalances. Key indicators of concern include elevated blood sodium, critically low levels of blood phosphorus and albumin, which are crucial for renal function and overall metabolic health. These factors, combined with the patient's advanced age and the critical nature of his condition, underscore the urgent need for comprehensive management and monitoring.
 \\

5. You need to consider the leader expert's opinion carefully and provide your opinion on the summary report generated by the leader expert. Please output the following two contents in JSON format:
(1) Your viewpoint on the opinion of the leader expert, i.e., the patient's risk is either high or low, respond with "agree" or "disagree".
(2) The confidence level of your opinion, respond with a number between 0 and 1.
(3) The reason for your opinion.
(4) If you disagree, the evidence you used to support your opinion. Please choose from the medical knowledge I provide as your evidence.\\

5. Here are two examples of the format you should output:
{"Answer": "agree", "Confidence": 0.8, "Reason": "The reason for your opinion."}
{"Answer": "disagree", "Confidence": 0.2, "Reason": "The reason for your opinion.", "Evidences": ["Evidence 1 ...", "Evidence 2 ..."]} \\

6. Respond in JSON format without any additional content: \\

\end{tcolorbox}

==> prompts/complete_prompts/collaborative_summary.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's Revised Summary Report: \\

1. You are an authoritative expert in the medical field. You are organizing a collaborative consultation. Now several doctors have made analysis and judgments on a patient's condition. Your task is to analyze the rationality of each doctor's opinion and summarize the opinions you think are reasonable to obtain a summary report for the patient. \\

2. In the previous discussion, you took into account the opinions of all the doctors and obtained a summary report about the patient, which is listed as follows:
In my opinion, the patient has a high risk of mortality.
The patient, a 59-year-old female with End-Stage Renal Disease due to chronic glomerulonephritis, exhibits several critical health indicators that suggest a high risk of mortality. Key concerns include significantly low systolic and diastolic blood pressures, critically low albumin levels indicating malnutrition or severe illness, and potential electrolyte imbalances as evidenced by low blood chlorine levels. These factors, coupled with her renal failure, contribute to a precarious health status.
 \\

3. Then, all the doctors offer new perspectives and opinions on your summary report. \\


4. In each doctor's statement, they first expressed whether they agreed with your statement in the previous summary report and gave the degree of confidence in their own judgment. Then, they further elaborated on their views by stating reasons and listing relevant literature.
The following are their opinions:
Doctor 0's statement is as following:
He thinks the mortality risk of the patient is: 0.00.
He first briefly analyzed the patient's basic condition: The patient, a 44-year-old male with End-Stage Renal Disease (ESRD) due to chronic glomerulonephritis, shows a low mortality risk as per the AdaCare model. Key indicators such as hemoglobin, blood sodium, and carbon dioxide binding power are within or close to the normal ranges, suggesting stable metabolic and renal functions. The patient's creatinine levels, indicative of kidney function, are consistently high, which is expected in ESRD. The slight deviations in blood sodium and carbon dioxide binding power from the average values of survival patients are minor and do not suggest significant health risks. Overall, the patient's condition appears to be managed well, with no acute exacerbations noted in the recent data provided.
Then, he listed some evidence as the basis for my diagnosis of this patient: Document [3] (Title: Anemia of Renal Disease - Hematology and Oncology - MSD Manual Professional Edition) discusses the normocytic and normochromic anemia often seen in chronic renal disease, which is consistent with the patient's hemoglobin levels being within the normal range.
Document [4] (Title: Medical Aspects of Long-Term Renal Replacement Therapy - Genitourinary Disorders - MSD Manual Professional Edition) highlights the importance of managing metabolic abnormalities in long-term RRT patients, which includes monitoring and maintaining electrolyte balance, as seen in the patient's stable blood sodium levels.
Document [15] (Title: Overview of Renal Replacement Therapy - Genitourinary Disorders - MSD Manual Professional Edition) emphasizes the need for continuous monitoring and management of ESRD patients, which supports the patient's ongoing stability and low mortality risk.
Doctor 1's statement is as following:
...... \\

5. You need to consider all the doctors' new ideas and modify your original summary report.
(1) If a doctor expresses strong opposition to your previous statement, you need to focus on his reasons and arguments and think carefully about whether you need to reconsider mortality risk of the patient and modify your summary report accordingly.
(2) If a doctor expresses opposition but also has some doubts about his own opinion, you need to consider his opinion, but you can stick to your original opinion.
(3) If a doctor expresses agreement, then you do not need to modify your original summary based on his opinion. \\ 

6. Please output the following three contents in JSON format:
(1) Your statement of mortality risk of the patient.
(2) Your revised summary report. Please create a concise and clear summary of the patient's health status. Your summary should be informative and beneficial for healthcare prediction tasks, such as in-hospital mortality prediction.
(3) Your reasons for revision in JSON format. The format of the reason for revision is: which doctor's opinion or relevant literature did you refer to, and which original opinion did you modify.

7. Here is an example of the revised summary report:
35-year-old female was diagnosed with chronic glomerulonephritis five years ago. Chronic kidney disease progressed to end stage renal disease (ESRD) over last year. Client was started on automated peritoneal dialysis six months ago. She developed fever, vomiting, and abdominal pain 1 day ago. Current assessment: T 39.1 °C, (102.40 F), HR 104, RR 16, B/P 145/ 87 mmHg. Weight: 66.8 Kg/147 lbs. NKDA. Periumbilical tenderness, defense and rebound. Erythema and creamy, yellow exudate around peritoneal dialysis catheter exit site. Dialysate effluent is cloudy yellow. Peritoneal effluent culture was obtained. Labs sent. The patient's complex medical history and the presence of multiple comorbidities suggest a high risk for in-hospital mortality. Close monitoring and management of these conditions are critical for patient outcomes. \\

8. Here are two examples of the format you should output:
{"Answer": "In my opinion, the patient has a high risk of mortality.", "Report": "...", "Reasons": ["reason1 ...", "reason2 ..."]}
{"Answer": "In my opinion, the patient has a low risk of mortality.", "Report": "...", "Reasons": ["reason1 ...", "reason2 ..."]} \\

9. Respond in JSON format without any additional content: \\

\end{tcolorbox}

==> prompts/complete_prompts/initial_doctor_review.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Doctors' Initial Review: \\

1. You are a helpful medical expert with extensive medical knowledge. I will provide you with electronic health record data for a patient, as well as some AI model analyses for this patient, including death risk prediction results and feature importance weight. The greater the feature importance weight, the greater the impact of that feature on the patient's outcome. When the patient's risk of death is low, this impact is positive; conversely, when the risk is high, the impact is negative. I will also retrieve relevant medical knowledge based on the AI model's analysis results and provide it to you. Please summarize the patient's condition based on the above information and generate an analytical report. \\

2. Here is the relevant medical knowledge:
Document [0] (Title: Diabetic Nephropathy - Genitourinary Disorders ...
Document [1] (Title: Understanding Medical Tests and Test Results ... 
... \\

3. Here is the healthcare context, including the patient's basic information and analysis results of AI models:

This male patient, aged 65.73, is an End-Stage Renal Disease(ESRD) patient with original disease Diabetic Nephropathy, and basic disease Diabetes.

Here is complete medical information from multiple visits of a patient, with each feature within this data as a string of values separated by commas.
- Blood chlorine: "1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0"
- Carbon dioxide binding power: "0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25"
......

The mortality prediction risk for the patient from AdaCare model is 0.01 out of 1.0, which means the patient is at a low level of death risk. Our model especially pays great attention to following features:
Carbon dioxide binding power: with shap value of 0.165. The feature value is 27.2 mmol/L, which is 1.0\% lower than the average value of survival patients (27.39 mmol/L), 1.0\% lower than the average value of deceased patients (27.42 mmol/L).
 The reference range is 20 mmol/L to 29 mmol/L.
Blood sodium: with shap value of 0.048. The feature value is 133.0 mmol/L, which is 4.0\% lower than the average value of survival patients (138.66 mmol/L), 3.0\% lower than the average value of deceased patients (137.27 mmol/L).
 The reference range is 135 mmol/L to 145 mmol/L.
Hemoglobin: with shap value of 0.025. The feature value is 149.0 g/L, which is 30.0\% higher than the average value of survival patients (114.98 g/L), 33.0\% higher than the average value of deceased patients (112.14 g/L).
 The reference range is 115 g/L to 150 g/L. \\

4. You need to analyze the patient's condition based on the above information and generate an analytical report. Please output the following contents in JSON format:
(1) The patient's death risk from AI model, just respond with a two-decimal number.
(2) Your analysis of the patient's condition.
(3) Choose reasonable evidence from the medical knowledge I provide to support your analysis. \\

5. Here is an example of the format you should output:
{"Logit": "0.73", "Analysis": "Your analysis of the patient's condition.", "Evidences": ["Evidence 1 ...", "Evidence 2 ..."]} \\

6. Respond in JSON format without any additional content:


\end{tcolorbox}

==> prompts/complete_prompts/initial_expert.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's Initial Summary Report: \\

1. You are an authoritative expert in the medical field. You are organizing a collaborative consultation. Now several doctors have made analysis and judgments on a patient's condition. Your task is to analyze the rationality of each general doctor's opinion, summarize the opinions you think are reasonable to obtain a summary report for the patient and give your judgment on the patient's mortality risk. \\

2. First, please read the patient's basic information carefully, as follows:
This male patient, aged 65.73, is an End-Stage Renal Disease(ESRD) patient with original disease Diabetic Nephropathy, and basic disease Diabetes.
 \\

3. Then, all doctors make a diagnosis on the patient's condition and give their reasons.
In each doctor's statement, they first analyze the important features they believe to be related to the patient's condition, then make a prediction about the mortality risk of the patient. Lastly, they collect and sort out relevant literature as evidence for their judgment.
The following are their opinions:

Doctor 0's statement is as following:
He thinks the mortality risk of the patient is: 0.01.
He first briefly analyzed the patient's basic condition: The patient, a 65-year-old male with End-Stage Renal Disease due to Diabetic Nephropathy and Diabetes, shows a low mortality risk as per the AdaCare model. Key indicators such as carbon dioxide binding power, blood sodium, and hemoglobin are within or close to the normal ranges, suggesting stable metabolic and renal functions. The patient's hemoglobin levels are notably higher than average, which could indicate better oxygen-carrying capacity and overall health status. However, fluctuations in weight and food intake suggest potential issues with nutritional management and fluid balance, which should be monitored closely to prevent complications.
Then, he listed some evidence as the basis for my diagnosis of this patient: Diabetic Nephropathy is the most common cause of end-stage kidney disease in the United States, accounting for up to 80\% of cases. The prevalence of renal failure is probably about 40\% among patients with type 1 diabetes mellitus. (Document [0])
Maintenance of glycosylated Hb (HbA1C) ≤ 7.0 is crucial for the treatment of Diabetic Nephropathy. Blood glucose control is primary treatment, and strict glucose control to maintain HbA1C ≤ 7.0; maintenance of euglycemia reduces microalbuminuria but may not retard disease progression once diabetic nephropathy is well-established. (Document [0])
Hyperphosphatemia, a consequence of phosphate retention due to low glomerular filtration rate (GFR), increases risk of soft-tissue calcification, especially in coronary arteries and heart valves, when calcium (Ca) × phosphate (PO4) > 55 mg2/dL2 (4.4 mmol2/L2). (Document [7])

Doctor 1's statement is as following:
......
 \\

4. You need to read all doctors' opinions carefully and analyze whether their opinions make sense and whether they are helpful in diagnosing the patient's condition. \\

5. Next, please write a summary report including the following:
1. A direct statement: in your opinion, whether the mortality risk of the patient is higher or not.
2. A summary of the patient's condition and the characteristics of the patient that you think are worthy of attention.
3. List of supporting evidence: [Doctor 0's opinion or relevant literature retrieved, Doctor 1's opinion or relevant literature retrieved, ...]. \\

6. Here are two examples of the format you should output:
{"Answer":"In my opinion, the patient has a high risk of mortality.", "Report": "...", "Evidences": ["Doctor 0's ... ", "Doctor 1's ..."]}.
{"Answer":"In my opinion, the patient has a low risk of mortality.", "Report": "...", "Evidences": ["Doctor 0's ... ", "Doctor 1's ..."]}. \\

7. Respond in JSON format without any additional content \\


\end{tcolorbox}

==> prompts/simple_prompts/action.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's decision of next action: \\

1. In response to the patient's summary report, several general doctors put forward their own opinions and reasons. 
In each general doctor's statement, they first expressed whether they agreed with the previous summary report and gave the degree of confidence in their own judgment. Then, they further elaborated on their views by stating reasons and listing relevant literature. 
The following are their opinions:
Doctor 0's statement is as following:
Regarding the summary report of the leader expert, I agree with the leader, with high confidence.
The reason to support my statement is announced below:
The patient's condition, as described in the summary report, aligns with the high-risk profile for mortality in patients with End-Stage Renal Disease due to Diabetic Nephropathy...
Doctor 1's statement is as following: ...
Doctor 2's statement is as following: ...
 \\

2. Next, you need to judge whether the next round of discussion is needed based on each general doctor's statement. Considering the following four cases:
(1) If all doctors agree with the previous summary report, there is no need to continue the discussion.
(2) If some doctors disagree with the previous report, but they are not confident in their judgment and have not listed convincing evidence, there is no need to continue the discussion.
(3) If some doctors strongly oppose the previous report and you think their evidence is worth discussing, we need to continue the discussion.
(4) If most doctors disagree with the previous report, we need to continue the discussion. \\

3. Please output the following two contents in JSON format:
(1) Whether to continue the discussion or not.
(2) Explain the reasons for your judgment. \\

\end{tcolorbox}

==> prompts/simple_prompts/collaborative_doctor_review.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Doctors' Discussion Review: \\


1. Here is the relevant medical knowledge:
Document [0] (Title: Hemodialysis ...
Document [1] (Title: ...
\\

2. Here is your initial analysis of the patient, which is not completely reasonable, and you may need to adjust it based on the leader expert's opinion:
{{analysis}} \\

2. Here is the opinion of the leader expert:
In my opinion, the patient has a high risk of mortality. \\

3. Here is the summary report generated by the leader expert:
The patient, a 65-year-old male with End-Stage Renal Disease due to Diabetic Nephropathy and Diabetes, exhibits significant clinical markers of severe renal dysfunction and metabolic imbalances. Key indicators of concern include elevated blood sodium, critically low levels of blood phosphorus and albumin, which are crucial for renal function and overall metabolic health. These factors, combined with the patient's advanced age and the critical nature of his condition, underscore the urgent need for comprehensive management and monitoring.
 \\

4. You need to consider the leader expert's opinion carefully and provide your opinion on the summary report generated by the leader expert. Please output the following two contents in JSON format:
(1) Your viewpoint on the opinion of the leader expert, i.e., the patient's risk is either high or low, respond with "agree" or "disagree".
(2) The confidence level of your opinion, respond with a number between 0 and 1.
(3) The reason for your opinion.
(4) If you disagree, the evidence you used to support your opinion. Please choose from the medical knowledge I provide as your evidence.\\


\end{tcolorbox}

==> prompts/simple_prompts/collaborative_summary.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's Revised Summary Report: \\

1. In the previous discussion, you took into account the opinions of all the doctors and obtained a summary report about the patient, which is listed as follows:

In my opinion, the patient has a high risk of mortality.
The patient, a 59-year-old female with End-Stage Renal Disease due to chronic glomerulonephritis, exhibits several critical health indicators that suggest a high risk of mortality. Key concerns include significantly low systolic and diastolic blood pressures, critically low albumin levels indicating malnutrition or severe illness,...
 \\

2. Then, all the doctors offer new perspectives and opinions on your summary report. \\

3. In each doctor's statement, they first expressed whether they agreed with your statement in the previous summary report and gave the degree of confidence in their own judgment. Then, they further elaborated on their views by stating reasons and listing relevant literature.

The following are their opinions:

Doctor 0's statement is as following:

He thinks the mortality risk of the patient is: 0.00.

He first briefly analyzed the patient's basic condition: The patient, a 44-year-old male with End-Stage Renal Disease (ESRD) due to chronic glomerulonephritis, shows a low mortality risk ... 
Then, he listed some evidence as the basis for my diagnosis of this patient: 
Document [3] (Title: Anemia of Renal Disease ...
Document [4] (Title: Medical Aspects ...
Document [15] ...

Doctor 1's statement is as following:
...... \\

4. You need to consider all the doctors' new ideas and modify your original summary report. Please output the following three contents in JSON format:
(1) Your statement of mortality risk of the patient.
(2) Your revised summary report. Please create a concise and clear summary of the patient's health status. Your summary should be informative and beneficial for healthcare prediction tasks, such as in-hospital mortality prediction.
(3) Your reasons for revision in JSON format. The format of the reason for revision is: which doctor's opinion or relevant literature did you refer to, and which original opinion did you modify.

5. Here is an example of the revised summary report:
35-year-old female was diagnosed with chronic glomerulonephritis five years ago. Chronic kidney disease progressed to end stage renal disease (ESRD) over last year. Client was started on automated peritoneal dialysis six months ago. She developed fever, vomiting, and abdominal pain 1 day ago. Current assessment: T 39.1 °C, (102.40 F), HR 104, RR 16, B/P 145/ 87 mmHg. Weight: 66.8 Kg/147 lbs. NKDA. Periumbilical tenderness, defense and rebound. Erythema and creamy, yellow exudate around peritoneal dialysis catheter exit site... \\


\end{tcolorbox}

==> prompts/simple_prompts/initial_expert.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=An example of a complete prompt template adopting the chain-of-thought strategy, 
    colframe=darkgray, 
    colback=white, 
    breakable]

Example Prompt Template of Expert's Initial Summary Report: \\


1. First, please read the patient's basic information carefully, as follows:
This male patient, aged 65.73, is an End-Stage Renal Disease(ESRD) patient with original disease Diabetic Nephropathy, and basic disease Diabetes.
 \\

2. Then, all doctors make a diagnosis on the patient's condition and give their reasons.
In each doctor's statement, they first analyze the important features they believe to be related to the patient's condition, then make a prediction about the mortality risk of the patient. Lastly, they collect and sort out relevant literature as evidence for their judgment.
The following are their opinions:

Doctor 0's statement is as following:
He thinks the mortality risk of the patient is: 0.01.
He first briefly analyzed the patient's basic condition: The patient, a 65-year-old male with End-Stage Renal Disease due to Diabetic Nephropathy and Diabetes, shows a low mortality risk as per the AdaCare model...

Then, he listed some evidence as the basis for my diagnosis of this patient: Diabetic Nephropathy is the most common cause of end-stage kidney disease in the United States, accounting for up to 80\% of cases. The prevalence of renal failure is probably ...

Doctor 1's statement is as following:
......
 \\

3. You need to read all doctors' opinions carefully and analyze whether their opinions make sense and whether they are helpful in diagnosing the patient's condition. \\

4. Next, please write a summary report including the following:
1. A direct statement: in your opinion, whether the mortality risk of the patient is higher or not.
2. A summary of the patient's condition and the characteristics of the patient that you think are worthy of attention.
3. List of supporting evidence: [Doctor 0's opinion or relevant literature retrieved, Doctor 1's opinion or relevant literature retrieved, ...]. \\

\end{tcolorbox}

==> prompts/simple_prompts/initial_review.tex <==
\begin{tcolorbox}[nobeforeafter, 
    title=Example Prompt Template of Doctors' Initial Review:, 
    colframe=darkgray, 
    colback=white, 
    breakable]
 \\
1. Here is the relevant medical knowledge:
Document [0] (Title: Diabetic Nephropathy - Genitourinary Disorders ...
Document [1] (Title: Understanding Medical Tests and Test Results ... 
... \\
2. Here is the healthcare context, including the patient's basic information and analysis results of AI models:\\
This male patient, aged 65.73, is an End-Stage Renal Disease(ESRD) patient with original disease Diabetic Nephropathy, and basic disease Diabetes.

Here is complete medical information from multiple visits of a patient, with each feature within this data as a string of values separated by commas.
- Blood chlorine: "1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0"
- Carbon dioxide binding power: "0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25, 0.25"
......

The mortality prediction risk for the patient from AdaCare model is 0.01 out of 1.0. Our model especially pays great attention to following features:
Carbon dioxide binding power: with shap value of 0.165. The feature value ...
Blood sodium: with shap value of 0.048. The feature value ...
Hemoglobin: with shap value of 0.025. The feature value... \\

3. You need to analyze the patient's condition based on the above information and generate an analytical report. Please output the following contents in JSON format:
(1) The patient's death risk from AI model, just respond with a two-decimal number.
(2) Your analysis of the patient's condition.
(3) Choose reasonable evidence from the medical knowledge I provide to support your analysis. \\


\end{tcolorbox}
